Systematic review and characterisation of malicious industrial network traffic datasets

The adoption of the Industrial Internet of Things (IIoT) as a complementary technology to Operational Technology (OT) has enabled a new level of standardised data access and process visibility. This convergence of Information Technology (IT), OT, and IIoT has also created new cybersecurity vulnerabilities and risks that must be managed. Artificial Intelligence (AI) is emerging as a powerful tool to monitor OT/IIoT networks for malicious activity and is a highly active area of research. AI researchers are applying advanced Machine Learning (ML) and Deep Learning (DL) techniques to the detection of anomalous or malicious activity in network traffic. They typically use datasets derived from IoT/IIoT/OT network traffic captures to measure the performance of their proposed approaches. Therefore, there is a widespread need for datasets for algorithm testing. This work systematically reviews publicly available network traffic capture-based datasets, including categorisation of contained attack types, review of metadata, and statistical as well as complexity analysis. Each dataset is analysed to provide researchers with metadata that can be used to select the best dataset for their research question. This results in an added benefit to the community as researchers can select the best dataset for their research more easily and according to their specific Machine Learning goals.

==> latexFeatureTable.tex <==
\begin{landscape}

\begin{table}[htp]
\centering
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{r c c c c c c c c c c }
   \multicolumn{1}{c}{\textbf{Dataset}} &  \multicolumn{10}{c}{Feature Number (ordered by importance)} \\
  \multicolumn{1}{c}{Complexity} & 1 &2 &3 &4 & 5& 6& 7&8 &9 & 10\\\hline\hline

\multicolumn{1}{c}{\textbf{HDGM}} & \includegraphics[width=0.15\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.15\textwidth,draft]{Feature01a.png}& & & & & & & &  \\ \hline


\multicolumn{1}{c}{\textbf{IEC 60780-5-104}} & \includegraphics[width=0.15\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.15\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.15\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.15\textwidth,draft]{Feature01a.png}& & & & & &  \\ \hline


\multicolumn{1}{c}{\textbf{DNP3}} & \includegraphics[width=0.15\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.15\textwidth,draft]{Feature01a.png}&\includegraphics[width=0.15\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.15\textwidth,draft]{Feature01a.png} & \includegraphics[width=0.15\textwidth,draft]{Feature01a.png}& & & & & &  \\ \hline




% 01 & {Flow\_IAT\_Min}	 
% \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}&  	 
% {Bwd\_Header\_Len}	 
% \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  {DLpkt\_Len\_MAX}\ \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
% 02 & \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
% 03 & \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
% 04 & \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
% 05 & \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
% 06 & \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
% 07 & \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
% 08 & \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
% 09 & \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
% 10 & \includegraphics[width=0.25\textwidth,draft]{Feature01a.png}& \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} &  \includegraphics[width=0.25\textwidth,draft]{Feature01a.png} \\\hline
\end{tabular}
\caption{Individual feature plots showing the distribution of benign (blue) and malicious (red) traffic for the ten most important features of each dataset. The horizontal axis of each plot is the row (or data point) index in the analysed CSV file and the vertical axis is the feature value on a linear scale from the feature’s minimum to its maximum value.}
\label{tab:mostimportant}
\end{table}


\end{landscape}
